Learning to Observe: Approximating Human Perceptual Thresholds for Detection of Suprathreshold Image Transformations

Many tasks in computer vision are often calibrated and evaluated relative to human perception. In this paper, we propose to directly approximate the perceptual function performed by human observers completing a visual detection task. Specifically, we present a novel methodology for learning to detect image transformations visible to human observers through approximating perceptual thresholds. To do this, we carry out a subjective two-alternative forced-choice study to estimate perceptual thresholds of human observers detecting local exposure shifts in images. We then leverage transformation equivariant representation learning to overcome issues of limited perceptual data. This representation is then used to train a dense convolutional classifier capable of detecting local suprathreshold exposure shifts - a distortion common to image composites. In this context, our model can approximate perceptual thresholds with an average error of 0.1148 exposure stops between empirical and predicted thresholds. It can also be trained to detect a range of different local transformations.

==> drafts.tex <==

Detection of image manipulations is an important area in computer vision, used in a variety of applications.

In this work we try to detect specific types of image manipulations associated with image composites.

The most common manipulations applied in the image compositing process are 2D point operators, specifically, brightness, contrast, hue and saturation (Xue). 

In manual compositing the application of these operations is often enough to significantly reduce the visible differences between the composite background and foreground elements, due to the limited sensitivity of the HVS.

Inferring both the location and parameter value of such point operators would enable us to identify regions of composites that have undergone particular processing with respect to the background, and provide us with a starting point to minimise these differences and improve the quality of a given composite. 

In this paper we present a CNN architecture for detection of brightness and contrast manipulations applied to regions of images drawn from the COCO dataset. We evaluate multiple state-of-the-art CNN architectures and motivate our choices for those. 

Related work:
- Saliency detection
- Semantic segmentation
- manipulation detection

Justification:
- Why learn parametric transformations and not composites? - we can appropriately control the amount of change and collect perceptual data
- 


EXPERIMENTS:

1. Manipulation parameter prediction on COCO
2. Fine-tuning a dense classifier based on perceptual thresholds
3. Classifier + AET

==> snippets.tex <==
Thus, creation of subjective quality models for CQA relies on the ability to approximate both spatial locations and parameters of such transformations and mapping those to empirical subjective quality scores.

The two fundamental differences between IQA and CQA are the \textit{feature space} images are represented in and the feature \textit{pooling strategy}. For example, NR IQA is often formulated as a weighted average of predicted quality scores for individual regions of an image, where the weighting corresponds to some saliency model, predicting allocation of attention and relative importance of different parts of the image to the overall quality function \cite{bosse2017deep}. These features correspond to global image properties that an observer is assumed to implicitly aggregate and weigh before assigning a quality score. In a different approach \cite{hou2014blind}, Natural Scene Statistics (NSS) are used to embed images in feature space, which are then classified images into 5 ordinal semantic quality categories, corresponding loosely to the Likert scale ratings often employed in subjective IQA tasks, and using the mean of the probability distribution across the 5 classes as a final numerical quality score. Other methods, such as \cite{talebi2018nima} extend prediction of the \textit{mean} quality score to prediction of the corresponding distribution of human quality scores, however none of these approaches tackle the problem of image composites directly, with the exception of the CNN-based model presented in \cite{zhu2015learning}. This model achieves state-of-the-art performance on binary classification of images into composites and real images, based on synthetically-generated composite images, however its discriminative nature and global response are both limiting factors for our application. 

In contrast to the above, CQA relies on finding local discontinuities in some feature space, indicating the presence of two regions from images generated/captured under disparate environmental conditions. The quality of $I_{fg}$ is thus dependant on the feature distribution of $I_{bg}$ -- if $I_{bg}$ was captured under brighter illumination, the previously adequate distribution $I_{fg}$ would yield a lower score. Thus, NR CQA can be expressed as a FR IQA problem posed within a single image (assuming $M_{fg}$ is known), where the background pixels act as a reference for the foreground element pixels. This means that the overall quality can be expressed as proportional to the inverse of differences between some feature representations of the $fg$ and $bg$ regions in an image, rather than a weighted sum, as in the case of IQA. 

$$Q(C(I_{fg}, I_{bg}; M_{fg})) \propto \frac{1}{||\phi(I_{fg}) - \phi(I_{bg})||}$$

Here, $Q$ is the image composite quality score, $\phi$ is a task-specific nonlinear transformation. In this feature space, unrealistic combinations of $I_{fg}$ and $I_{bg}$ yield high spatial discontinuities:

$$\sigma^2(\phi(I_{real})) < \sigma^2(\phi(I_{comp}))$$

Thus, the CQA task relies on approximating $\phi$, such that the difference between predicted and ground truth composite quality scores is minimised. This could be achieved using deep learning, provided the existence of a large enough labelled dataset. Unfortunately, most tasks involving humans and collection of subjective opinions are expensive and time-consuming endeavours, particularly at scale. Because an image composite can combine elements from multiple real images, even those which could not realistically occur together in a single natural image, this problem compounds further. This makes it challenging to gather plausible composite images in large quantities and screen them against a large enough corpus of human observers in order to generalize well for unseen images.  

Recent deep learning-based approaches have been able to significantly improve on the global IQA task over their predecessors. In \cite{bosse2017deep} the authors propose a convolutional neural network (CNN) which predicts a global quality score by weighting local quality estimates learned from randomly sampled image patches using an attention branch. Sadly, these techniques are conditioned on artifacts commonly associated with global quality, such as compression artifacts, blur or noise, rendering them inappropriate for CQA applications.

% Maybe some more approaches and why they are incompatible here...

In this paper we propose an efficient, semi-supervised approach to encoding image features relevant to compositing operations, which extends the Auto-Encoding Transformation (AET) approach \cite{zhang2019aet}

https://arxiv.org/pdf/1803.11395.pdf
https://arxiv.org/pdf/1803.11395.pdf
https://arxiv.org/pdf/1803.11395.pdf
https://arxiv.org/pdf/1803.11395.pdf

https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=8451698

http://openaccess.thecvf.com/content_cvpr_2016/papers/Niu_Ordinal_Regression_With_CVPR_2016_paper.pdf
https://www.cv-foundation.org/openaccess/content_cvpr_2015/papers/Li_Visual_Saliency_Based_2015_CVPR_paper.pdf

% In contrast, image composite quality can be seen as a function of visible differences between the sets of features of the background and foreground elements. If we assume the foreground element is appropriately spatially transformed such that its placement against the background appears plausible, then the quality of this combination can be defined as a function of:


% $$Q(I_{bg}, I_{fg}) = \frac{1}{n}\sum_{i=1}^{n}{w_{(i)}T(||\phi{(x_{bg})}_{(i)} - \phi{(x_{fg})}_{(i)}||)},$$


% where $x_{bg}$ and $x_{fg}$ are the background and foreground image regions of $x$ respectively, $\phi(x)_{i}$ is the $i$th feature vector resulting from a nonlinear transformation  $T$ is a perceptual threshold function, indicating whether the magnitude of a given feature disparity is above the perceptual threshold and $w$ is the perceptual weighting of the visible feature.




% Due to the abundance of compositing and synthesis tools, local measures of image quality are necessary both for aiding humans, as well as automatic identification of image regions of low enough quality for an average observer to notice. 

% Talk about how to learn $\phi$ without sufficient data. Maybe move the threshold term to parameters?

% use references from the compositing paper regarding definitIn ions of composites

% Mention AET and learning transformations here.


% \textbf{THE ESSENCE: We show how we can first learn a representation of a particular feature disparity in an unsupervised manner and then perceptually tune it using a smaller dataset.}
% https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=7139092
% https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=7139092
% https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=7139092



In order to detect instances of local suprathreshold pixel intensity scaling, we propose to learn a TER in an unsupervised fashion, by adopting the AET paradigm to local pixel intensity transformations. We then train a supervised pixel-wise classifier to label each pixel as belonging to one of 3 classes: \textit{no suprathreshold offset}, \textit{positive suprathreshold offset}, \textit{negative suprathreshold offset}.

As discussed in the introduction, we formulate the CQA problem as detection of disparities between $I_{fg}$ and $I_{bg}$, followed by applying an empirical perceptual threshold $x_T = \Psi^{-1}(\pi_{T})$ calculated with respect to the type of disparity present. This perceptual threshold, along with the underlying psychometric function, tend to vary as a function of observer, image content and viewing conditions. We wish to capture the content-dependant variation, while minimising the impact of different observers. In order to achieve this, we pool observer thresholds for each image and boostrap a mean threshold value for each image. 

\subsection{Simplifying Assumptions}
In order to evaluate our proposed approach, we focus on a particular type of transformation -- pixel intensity scaling -- corresponding to modifying camera exposure. This is motivated by the fact that intensity scaling combines luminance and contrast changes: two highly correlated image statistics between foregrounds and backgrounds of natural images \cite{xue2012understanding}. In manual compositing, matching the luminance and contrast between the composite elements is commonly the first and most important step towards achieving a plausible result \cite{wright2013compositing}. Finally, naive observers can reliably detect such image manipulations \cite{dolhasz2016measuring, dolhasz2017poster}, which reduces the number of trials required to fit psychometric functions to experimental data using staircase methods such as QUEST \cite{watson1983quest}.

\subsection{Representation Learning}
As our model operates on natural images, we can leverage transfer learning techniques \cite{weiss2016survey} which use weights learned on classification tasks to initialise parameter values, before training on new task. The ImageNet Large Scale Visual Recognition Challenge 2010 is a popular source of pre-trained weights used in a range of natural-image-based applications \cite{marmanis2015deep, kornblith2019better}. These features have also been successfully leveraged in deep similarity metrics \cite{zhang2018unreasonable}, showing significant correlation between representations learned by these networks and human perceptual judgements. While these representations can be useful starting points for a range of tasks, if the target task is sufficiently different from the source task and the target dataset is too small, the results may be suboptimal. Furthermore, if the networks have been trained for very different tasks within the same domain, only layers closer to the input learn useful features, while deeper layers tend to learn task-specific features, irrelevant for the transfer task \cite{geirhos2018imagenet}. In order to leverage ImageNet weights, while ensuring better performance on our task, we initialise our models from ImageNet weights, but perform an additional stage unsupervised training in order to learn a TER for our image adjustments. This allows us to use a large dataset such as MS COCO \cite{lin2014microsoft}.

